Structured Credal Learning

Real-world learning tasks often encounter uncertainty due to covariate shift and noisy or inconsistent labels. However, existing robust learning methods merge these effects into a single distributional uncertainty set. In this work, we introduce a novel structured credal learning framework that explicitly separates these two sources. Specifically, we derive geometric bounds on the total variation diameter of structured credal sets and demonstrate how this quantity decomposes into contributions from covariate shift and expected label disagreement. This decomposition reveals a gating effect: covariate modulates how much label disagreement contributes to the joint uncertainty, such that seemingly benign covariate shifts can substantially increase the effective uncertainty. We also establish finite-sample concentration bounds in a fixed covariate regime and demonstrate that this quantity can be efficiently estimated. Lastly, we show that robust optimization over these structured credal sets reduces to a tractable discrete min-max problem, avoiding ad-hoc robustness parameters. Overall, our approach provides a principled and practical foundation for robust learning under combined covariate and label mechanism ambiguity.

==> chapters/2_background.tex <==

\paragraph{Covariate shift~} Given input $x \in \mathcal{X}$, covariate shift refers to the setting in which the marginal input distribution differs between training and test time, $P_{\mathrm{train}}(X) \neq P_{\mathrm{test}}(X)$, while the conditional label distribution remains invariant, $P_{\mathrm{train}}(Y \mid X) = P_{\mathrm{test}}(Y \mid X)$. Under this assumption, the Bayes-optimal predictor is unchanged; however, empirical risk minimization becomes biased since the training objective estimates expectations with respect to $P_{\mathrm{train}}(X)$ rather than the target distribution $P_{\mathrm{test}}(X)$. Formally, the test risk
\[
\mathcal{R}_{\mathrm{test}}(f) = \mathbb{E}_{(X,Y) \sim P_{\mathrm{test}}}[\ell(f(X),Y)]
\]
can be expressed using importance weighting as
\[
    \mathcal{R}_{\mathrm{test}}(f) = \mathbb{E}_{(X,Y) \sim P_{\mathrm{train}}}\!\left[w(X)\,\ell(f(X),Y)\right],
\]
where $w(X) = \frac{P_{\mathrm{test}}(X)}{P_{\mathrm{train}}(X)}.$
This formulation highlights that learning under covariate shift requires correcting for discrepancies in the input distribution rather than modifying the conditional model $P(Y \mid X)$. 

\paragraph{Label uncertainty~} Given input $x \in \mathcal{X}$, label uncertainty refers to the setting in which the conditional label distribution $P(Y \mid X=x)$ is non-degenerate and potentially noisy, reflecting stochasticity, ambiguity, or measurement error in the data-generating process. Unlike covariate shift, the marginal input distribution may remain unchanged, while uncertainty arises from variability in the target conditional on the same input. In our framework, this ambiguity is quantified via total variation disagreement rather than entropy, since it directly controls the diameter of the structured credal set and the resulting robustness penalty. 
\[
\mathcal{R}(f) = \mathbb{E}_{(X,Y) \sim P}[\ell(f(X),Y)]
\]
therefore contains an irreducible component induced by disagreement in 
$P(Y \mid X)$ that cannot be removed by increasing the sample size. Addressing label uncertainty thus requires improving supervision quality or modeling annotator variability, rather than adapting the marginal feature distribution.



\iffalse

\paragraph{Distributionally Robust Optimization}
DRO replaces empirical risk minimization with a worst-case objective over a set of plausible data distributions. Formally, given a loss function $\ell:\mathcal{X}\times\mathcal{Y}\to\mathbb{R}_{+}$ and an uncertainty set $\mathcal{Q}$ of probability distributions over $\mathcal{X}\times\mathcal{Y}$, DRO solves:

\begin{equation}
\min_{\theta \in \Theta} \; \sup_{Q \in \mathcal{Q}} \; \mathbb{E}_{(x,y)\sim Q}\!\left[\ell(f_\theta(x), y)\right].
\label{eq:dro}
\end{equation}

The choice of $\mathcal{Q}$ determines the types of distributional shifts against which the learned model is robust. Common constructions define $\mathcal{Q}$ as a divergence-based neighborhood around the empirical training distribution, such as a Wasserstein or $f$-divergence ball, or as a convex hull of distributions associated with known data-generating environments. While such formulations provide worst-case guarantees, they often require ad-hoc specification of uncertainty radii and may lead to overly pessimistic solutions.

\fi


% STL and CTL limitations for sepration of these two sources of error
%However, classical statistical learning theory aggregates all variability into a single data-generating distribution, while credal learning theory~\cite{caprio2024credal,lohr2025credal} replaces this distribution with a convex set of plausible alternatives to obtain worst-case guarantees. Although this shift yields robustness to unspecified distributional changes, it treats heterogeneity in inputs and ambiguity in labeling mechanisms symmetrically, collapsing them into a single scalar robustness penalty. As a result, without explicit structural assumptions on how uncertainty arises, these theories provide no guidance on whether errors should be addressed through domain shift -- multi-source data collection, or reconciliation of conflicting labels. 

%\citet{} propose DIstribution Shift DEcomposition (DISDE), a diagnostic framework that decomposes performance loss into contributions from covariate shift (changes in $P_X$) and conditional shift (changes in $P_{Y∣X}$), further separating covariate effects into shared versus unseen or rare regions of the feature space~\cite{}. Their approach builds on ideas from causal inference and domain adaptation by defining a shared support distribution and estimating importance weights via an auxiliary domain classifier. In contrast,~\citet{} focus on uncertainty quantification under distribution shift, extending conformal prediction beyond the exchangeability assumption by explicitly modeling distinct roles of covariate shift and conditional shift ~\citep{}. They situate their work relative to robust conformal prediction methods that guard against worst-case joint shifts, arguing that such approaches can be overly conservative when shifts in $X$ and $Y|X$ are not disentangled.
%Methodologically, DISDE is a post-hoc diagnostic tool that attributes observed performance drops to interpretable components by reweighting training and test samples to a shared distribution and estimating counterfactual risks under fixed marginals or conditionals ~\cite{} . This decomposition is intended to guide targeted interventions such as reweighting, feature engineering, or new data collection. By contrast, the Weighted Robust Conformal Prediction (WRCP) framework explicitly reweights training samples to correct identifiable covariate shift while simultaneously inflating prediction quantiles to protect against worst-case conditional shift bounded by an f-divergence ball \citep{} . A doubly robust extension further mitigates errors in density-ratio estimation by combining outcome modeling and importance weighting. Together, these methods reflect a broader trend toward fine-grained treatment of distributional shifts: DISDE provides interpretability and diagnostic insight, whereas WRCP provides calibrated predictive uncertainty with formal coverage guarantees under structured shift assumptions.

==> chapters/tables/block.tex <==
\begin{table}[htbp]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\caption{Labeling mechanism complexity concentration bounds in the deterministic hard label regime (Block Method) under covariate distribution N(0,1). Fixed sample size $n = 1000$. Repetitions $R = 2000$. Here, $N_Y$ denotes the number of labeling mechanisms. $\widehat{p}_{\mathrm{viol}}$ is the estimated probability of violations. Let $\epsilon := \left|\eta_{Y|X}^\ast - \hat{\eta}_{Y|X}\right|$ and $q_{\alpha}(\epsilon)$ denote the empirical $\alpha$-quantile of $\epsilon$. The union Hoeffding bound is $\epsilon_{\mathrm{Hoeff}}^{\cup}$.}
\label{tab:b01}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{rrrrrrrr}
\toprule
$N_Y$ & $q_{0.5}(\epsilon)$ & $q_{0.95}(\epsilon)$ & $\epsilon_{\mathrm{Hoeff}}^{\cup}$ & $\widehat{p}_{\mathrm{viol}}$ & $\mathrm{CI}^{\mathrm{Wilson}}_{0.95,\mathrm{low}}$ & $\mathrm{CI}^{\mathrm{Wilson}}_{0.95,\mathrm{high}}$ & Tightness Ratio \\
\midrule
2 & 0.009 & 0.025 & 0.043 & 0.001 & 0.000 & 0.004 & 1.718 \\
5 & 0.015 & 0.032 & 0.055 & 0.000 & 0.000 & 0.002 & 1.710 \\
12 & 0.025 & 0.039 & 0.063 & 0.000 & 0.000 & 0.002 & 1.609 \\
20 & 0.029 & 0.042 & 0.067 & 0.000 & 0.000 & 0.002 & 1.591 \\
30 & 0.032 & 0.045 & 0.070 & 0.000 & 0.000 & 0.002 & 1.553 \\
50 & 0.035 & 0.048 & 0.073 & 0.000 & 0.000 & 0.002 & 1.531 \\
80 & 0.039 & 0.052 & 0.077 & 0.000 & 0.000 & 0.002 & 1.474 \\
100 & 0.040 & 0.052 & 0.078 & 0.000 & 0.000 & 0.002 & 1.502 \\
200 & 0.045 & 0.056 & 0.082 & 0.000 & 0.000 & 0.002 & 1.472 \\
500 & 0.050 & 0.061 & 0.088 & 0.000 & 0.000 & 0.002 & 1.440 \\
1000 & 0.053 & 0.064 & 0.092 & 0.000 & 0.000 & 0.002 & 1.432 \\
\bottomrule
\end{tabular}

\end{adjustbox}
\end{table}


==> chapters/tables/iv01.tex <==
\begin{table}[!htbp]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\caption{Labeling mechanism complexity concentration bounds in the deterministic hard label regime (Interval Method) under covariate distribution N(0,1). Fixed sample size $n = 1000$. Repetitions $R = 2000$. Here, $N_Y$ denotes the number of labeling mechanisms. $\widehat{p}_{\mathrm{viol}}$ is the estimated probability of violations. Let $\epsilon := \left|\eta_{Y|X}^\ast - \hat{\eta}_{Y|X}\right|$ and $q_{\alpha}(\epsilon)$ denote the empirical $\alpha$-quantile of $\epsilon$. The union Hoeffding bound is $\epsilon_{\mathrm{Hoeff}}^{\cup}$.}
\label{tab:iv01}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{rrrrrrrr}
\toprule
$N_Y$ & $q_{0.5}(\epsilon)$ & $q_{0.95}(\epsilon)$ & $\epsilon_{\mathrm{Hoeff}}^{\cup}$ & $\widehat{p}_{\mathrm{viol}}$ & $\mathrm{CI}^{\mathrm{Wilson}}_{0.95,\mathrm{low}}$ & $\mathrm{CI}^{\mathrm{Wilson}}_{0.95,\mathrm{high}}$ & Tightness Ratio \\
\midrule
2 & 0.007 & 0.021 & 0.043 & 0.000 & 0.000 & 0.002 & 2.085 \\
5 & 0.011 & 0.031 & 0.055 & 0.001 & 0.000 & 0.003 & 1.784 \\
12 & 0.010 & 0.030 & 0.063 & 0.000 & 0.000 & 0.002 & 2.095 \\
20 & 0.011 & 0.030 & 0.067 & 0.000 & 0.000 & 0.002 & 2.225 \\
30 & 0.010 & 0.029 & 0.070 & 0.000 & 0.000 & 0.002 & 2.392 \\
50 & 0.010 & 0.030 & 0.073 & 0.000 & 0.000 & 0.002 & 2.411 \\
80 & 0.011 & 0.031 & 0.077 & 0.000 & 0.000 & 0.002 & 2.465 \\
100 & 0.011 & 0.032 & 0.078 & 0.000 & 0.000 & 0.002 & 2.433 \\
200 & 0.011 & 0.032 & 0.082 & 0.000 & 0.000 & 0.002 & 2.570 \\
500 & 0.013 & 0.034 & 0.088 & 0.000 & 0.000 & 0.002 & 2.595 \\
1000 & 0.013 & 0.035 & 0.092 & 0.000 & 0.000 & 0.002 & 2.599 \\
\bottomrule
\end{tabular}

\end{adjustbox}
\end{table}


==> chapters/tables/iv02.tex <==
\begin{table}[!htbp]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\caption{Labeling mechanism complexity concentration bounds in the deterministic hard label regime (Interval Method) under covariate distribution N(0,2). Fixed sample size $n = 1000$. Repetitions $R = 2000$. Here, $N_Y$ denotes the number of labeling mechanisms. $\widehat{p}_{\mathrm{viol}}$ is the estimated probability of violations. Let $\epsilon := \left|\eta_{Y|X}^\ast - \hat{\eta}_{Y|X}\right|$ and $q_{\alpha}(\epsilon)$ denote the empirical $\alpha$-quantile of $\epsilon$. The union Hoeffding bound is $\epsilon_{\mathrm{Hoeff}}^{\cup}$.}
\label{tab:iv02}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{rrrrrrrr}
\toprule
$N_Y$ & $q_{0.5}(\epsilon)$ & $q_{0.95}(\epsilon)$ & $\epsilon_{\mathrm{Hoeff}}^{\cup}$ & $\widehat{p}_{\mathrm{viol}}$ & $\mathrm{CI}^{\mathrm{Wilson}}_{0.95,\mathrm{low}}$ & $\mathrm{CI}^{\mathrm{Wilson}}_{0.95,\mathrm{high}}$ & Tightness Ratio \\
\midrule
2 & 0.005 & 0.016 & 0.043 & 0.000 & 0.000 & 0.002 & 2.703 \\
5 & 0.010 & 0.028 & 0.055 & 0.000 & 0.000 & 0.002 & 1.928 \\
12 & 0.010 & 0.029 & 0.063 & 0.000 & 0.000 & 0.002 & 2.182 \\
20 & 0.010 & 0.029 & 0.067 & 0.000 & 0.000 & 0.002 & 2.323 \\
30 & 0.010 & 0.029 & 0.070 & 0.000 & 0.000 & 0.002 & 2.438 \\
50 & 0.011 & 0.030 & 0.073 & 0.000 & 0.000 & 0.002 & 2.428 \\
80 & 0.011 & 0.032 & 0.077 & 0.000 & 0.000 & 0.002 & 2.377 \\
100 & 0.012 & 0.033 & 0.078 & 0.000 & 0.000 & 0.002 & 2.349 \\
200 & 0.012 & 0.033 & 0.082 & 0.000 & 0.000 & 0.002 & 2.478 \\
500 & 0.013 & 0.036 & 0.088 & 0.000 & 0.000 & 0.002 & 2.428 \\
1000 & 0.013 & 0.035 & 0.092 & 0.000 & 0.000 & 0.002 & 2.607 \\
\bottomrule
\end{tabular}

\end{adjustbox}
\end{table}


==> chapters/tables/iv21.tex <==
\begin{table}[!htbp]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\caption{Labeling mechanism complexity concentration bounds in the deterministic hard label regime (Interval Method) under covariate distribution N(2,1). Fixed sample size $n = 1000$. Repetitions $R = 2000$. Here, $N_Y$ denotes the number of labeling mechanisms. $\widehat{p}_{\mathrm{viol}}$ is the estimated probability of violations. Let $\epsilon := \left|\eta_{Y|X}^\ast - \hat{\eta}_{Y|X}\right|$ and $q_{\alpha}(\epsilon)$ denote the empirical $\alpha$-quantile of $\epsilon$. The union Hoeffding bound is $\epsilon_{\mathrm{Hoeff}}^{\cup}$.}
\label{tab:iv21}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{rrrrrrrr}
\toprule
$N_Y$ & $q_{0.5}(\epsilon)$ & $q_{0.95}(\epsilon)$ & $\epsilon_{\mathrm{Hoeff}}^{\cup}$ & $\widehat{p}_{\mathrm{viol}}$ & $\mathrm{CI}^{\mathrm{Wilson}}_{0.95,\mathrm{low}}$ & $\mathrm{CI}^{\mathrm{Wilson}}_{0.95,\mathrm{high}}$ & Tightness Ratio \\
\midrule
2 & 0.003 & 0.009 & 0.043 & 0.000 & 0.000 & 0.002 & 4.605 \\
5 & 0.007 & 0.022 & 0.055 & 0.000 & 0.000 & 0.002 & 2.496 \\
12 & 0.008 & 0.022 & 0.063 & 0.000 & 0.000 & 0.002 & 2.820 \\
20 & 0.008 & 0.022 & 0.067 & 0.000 & 0.000 & 0.002 & 3.004 \\
30 & 0.008 & 0.022 & 0.070 & 0.000 & 0.000 & 0.002 & 3.226 \\
50 & 0.008 & 0.022 & 0.073 & 0.000 & 0.000 & 0.002 & 3.336 \\
80 & 0.008 & 0.022 & 0.077 & 0.000 & 0.000 & 0.002 & 3.409 \\
100 & 0.007 & 0.023 & 0.078 & 0.000 & 0.000 & 0.002 & 3.328 \\
200 & 0.007 & 0.022 & 0.082 & 0.000 & 0.000 & 0.002 & 3.825 \\
500 & 0.008 & 0.022 & 0.088 & 0.000 & 0.000 & 0.002 & 3.986 \\
1000 & 0.008 & 0.023 & 0.092 & 0.000 & 0.000 & 0.002 & 3.991 \\
\bottomrule
\end{tabular}

\end{adjustbox}
\end{table}

